Lagrangian Reachabililty

We introduce LRT, a new Lagrangian-based ReachTube computation algorithm that conservatively approximates the set of reachable states of a nonlinear dynamical system. LRT makes use of the Cauchy-Green stretching factor (SF), which is derived from an over-approximation of the gradient of the solution flows. The SF measures the discrepancy between two states propagated by the system solution from two initial states lying in a well-defined region, thereby allowing LRT to compute a reachtube with a ball-overestimate in a metric where the computed enclosure is as tight as possible. To evaluate its performance, we implemented a prototype of LRT in C++/Matlab, and ran it on a set of well-established benchmarks. Our results show that LRT compares very favorably with respect to the CAPD and Flow* tools.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

==> setting.tex <==
\section{Setting}
\label{sec:setting}
We consider the \emph{Cauchy problem} for non-autonomous \emph{ordinary differential equations} (ODEs)
\begin{subequations}
\label{cauchy}
\begin{align}
  x^\prime(t)&= F( t, x(t) ),\\
  x(t)&= x_0,
\end{align}
\end{subequations}
where $x\colon\mathbb{R}\to\mathbb{R}^n$. 
The vector field $F$ may depend on time, because our main interest lies in studying ODEs arising
in cardiac dynamics research, those models often include variables, which depend on time, e.g.
an excitation variable \textbf{ref.req.}.

Let $\phi\colon\mathbb{R}_+\times\mathbb{R}^n\to\mathbb{R}^n$ denotes the flow inducted by the dynamical system \eqref{cauchy}, i.e. 
$\phi_{t_0}^T(x_0)$ is the solution of \eqref{cauchy} with the initial condition $(t_0,x_0)$ at time $T$.
\newcommand{\rd}{\delta}

We present and implement an algorithm for computation of the continuous \emph{reach-tube} for
the provided Cauchy problem of the form \eqref{cauchy}. The algorithm is based on a computation of the gradient of the flow of \eqref{cauchy}, and then estimating the \emph{Cauchy-Green stretching factor} providing a rate of expansion of any two solutions in a set of initial conditions.

The motivation of the presented research is to develop a procedure enablingr a long-horizon time integration of \emph{cardiac dynamical systems}, and resulting in a tighter interval enclosures for the true solution curves of the problem under study compared to 
those obtained by available tools.
We hope that the proposed procedure will enable us to perform a long-horizon time integration of \emph{cardiac dynamical systems}. We expect an improvement over existing tools (described later), as we essentially compute an \emph{intersection} of results from several different available tools, such that the produced output is no worse than any of the results provided by the available tools. Moreover, we think that the outputted bounds are tighter, as the global stability exhibited generically by cardiac dynamics models is exploited by computation of the Cauchy-Green stretching factor.

To compute the gradient of the flow we use some of the available tools, including \emph{CAPD library} \cite{CAPD, Lo, ZW1, Z1}, and \emph{Flow*} \cite{CAS, CAS2}. Those libraries have been verified to provide a conservative results, guaranteeing that the outputted enclosures bound the true solution. For instance, the CAPD library have been used in many peer-reviewed computer proofs of theorems in dynamical systems, including \cite{GZ,TZ,WZ2}. Whereas, Flow* is based on the high-order Taylor models [BM98].

In Section~\ref{cgstreching}, we present the rigorous computation of the Cauchy-Green stretching factor. 
In Section~\ref{secrigcomp}, we present an algorithm performing the computation.

